On Reference (In-)Determinacy in Natural Language Inference

We revisit the reference determinacy (RD) assumption in the task of natural language inference (NLI), i.e., the premise and hypothesis are assumed to refer to the same context when human raters annotate a label. While RD is a practical assumption for constructing a new NLI dataset, we observe that current NLI models, which are typically trained solely on hypothesis-premise pairs created with the RD assumption, fail in downstream applications such as fact verification, where the input premise and hypothesis may refer to different contexts. To highlight the impact of this phenomenon in real-world use cases, we introduce RefNLI, a diagnostic benchmark for identifying reference ambiguity in NLI examples. In RefNLI, the premise is retrieved from a knowledge source (i.e., Wikipedia) and does not necessarily refer to the same context as the hypothesis. With RefNLI, we demonstrate that finetuned NLI models and few-shot prompted LLMs both fail to recognize context mismatch, leading to over 80% false contradiction and over 50% entailment predictions. We discover that the existence of reference ambiguity in NLI examples can in part explain the inherent human disagreements in NLI and provide insight into how the RD assumption impacts the NLI dataset creation process.

==> sections/acknowledgements.tex <==
\section*{Acknowledgements}
We thank Michael Collins, Corinna Cortes, Paul Haahr, Ilya Kornakov, Ivan Kuznetsov, Annie Louis, Don Metzler, Jeremiah Milbauer, Pavel Nalivayko, Fernando Pereira, Sandeep Tata, Yi Tay, Andrew Tomkins, and Victor Zaytsev for insightful discussions, suggestions, and support. We are grateful to the annotators for their work in creating \datasetname.

==> sections/limitations.tex <==
\section*{Limitations}
Since the \datasetname dataset feature entailment labels for \textit{all} propositions in a document, the label distribution are naturally imbalanced, which would potentially pose challenge for modeling. We observe low presence of contradiction examples in our dataset construction process, which could be a limiting factor for the utility of the dataset.
Unlike previous NLI datasets~\cite{bowman-etal-2015-large, williams-etal-2018-broad}, we speculate that reference determinacy, i.e. whether the hypothesis and premise refer to the same scenario at the same time, cannot be certainly guaranteed and safely assumed in our case, which in part leads to low presence of contradictions during annotation.
We offer a detailed discussion on the implications of reference determinacy and contradictions in Appendix~\ref{appendix:contradictions}. We leave the exploration on \emph{natural} contradictions for future work. 

As the annotation complexity and cost scales quadratically w.r.t. the number of propositions in a document, we truncate the documents in \datasetname to the first ten sentences of the original document. 

\section*{Ethical Considerations}
In the proposition-level entailment task ($T_2$), the inference of the entailment relation between a premise document and a hypothesis proposition uses the \emph{assumption} that the premise document is true. The assumption is common to NLI datasets \cite{dagan2005pascal, bowman-etal-2015-large, williams-etal-2018-broad}, and is necessary for the task's structure. With the documents in \datasetname, we make the assumption only for the experimental purpose of $T_2$, and make no claim about the actual veracity of the premise documents.

The full dataset will be released upon publication.

==> sections/pilot.tex <==
\section{A}
